AP-side WLAN Analytics

Monitoring the network performance experienced by the end-user is crucial for managers of wireless networks as it can enable them to remotely modify the network parameters to improve the end-user experience. Unfortunately, for performance monitoring, managers are typically limited to the logs of the Access Points (APs) that they manage. This information does not directly capture factors that can hinder station (STA) side transmissions. Consequently, state-of-the-art methods to measure such metrics primarily involve active measurements. Unfortunately, such active measurements increase traffic load and if used regularly and for all the STAs can potentially disrupt user traffic, thereby worsening performance for other users in the network and draining the battery of mobile devices. This thesis enables passive AP-side network analytics. In the first part of the thesis, I present virtual speed test, a measurement based framework that enables an AP to estimate speed test results for any of its associated clients solely based on AP-side observables. Next, I present Uplink Latency Microscope (uScope), an AP-side framework for estimation of WLAN uplink latency for any of the associated STAs and decomposition into its constituent components. Similar to virtual speed test, uScope makes estimations solely based on passive AP-side observations. We implement both frameworks on a commodity hardware platform and conduct extensive field trials on a university campus and in a residential apartment complex. In over 1 million tests, the two proposed frameworks demonstrate an estimation accuracy with errors under 10%.

==> secs/notation_def.tex <==

%\newglossaryentry{lengthtree}%
%{%
  %name={$L_t$},
  %text={L_t},
  %description={description here},
  %sort={L}
%}


\newglossaryentry{gM}%
{%
  name={$M$},
  text={M},
  description={Number of transmitter antennas.}
}

\newglossaryentry{gK}%
{%
  name={$K$},
  text={K},
  description={Number of receiving antennas.}
}

\newglossaryentry{gH}%
{%
  name={$H$},
  text={H},
  description={The MIMO CSI matrix.}
}

\newglossaryentry{gW}%
{%
  name={$W$},
  text={W},
  description={The MIMO steering weight matrix.},
}

\newglossaryentry{gPINV}%
{%
  name={$(\cdot )^\dagger$},
  text={(\cdot )^\dagger},
  description={The pseudo-inverse.},
}

\newglossaryentry{gIDEN}%
{%
  name={$I$},
  text={I},
  description={The identity matrix.},
}

\newglossaryentry{gC}%
{%
  name={$C$},
  text={C},
  description={Shannon Capacity (b/s/hz).}
}

\newglossaryentry{gRho}%
{%
  name={$\rho$},
  text={\rho},
  description={Correlation coefficient.}
}

\newglossaryentry{gDem}%
{%
  name={$d$},
  text={d},
  description={Demmel condition number.}
}

\newglossaryentry{gEV}%
{%
  name={$\lambda_k$},
  text={\lambda_k},
  description={The $k$th eigenvalue.}
}

\newglossaryentry{gSV}%
{%
  name={$\sigma_k$},
  text={\sigma_k},
  description={The $k$th singular value.}
}


\newglossaryentry{gh}%
{%
  name={$\vec{h}$},
  text={\vec{h}},
  description={A particular user's channel vector (row of $H$ matrix).}
}

\newglossaryentry{gw}%
{%
  name={$\vec{w}$},
  text={\vec{w}},
  description={A particular user's steering vector (column of $W$ matrix).}
}

\newglossaryentry{gP}%
{%
  name={$P$},
  text={P},
  description={Power allocated to a particular user.}
}



\newglossaryentry{gHerm}%
{%
  name={$(\cdot)^\textsc{H}$},
  text={(\cdot)^\textsc{H}},
  description={Hermetian transpose.}
}


